Fairness and Privacy Guarantees in Federated Contextual Bandits

This paper considers the contextual multi-armed bandit (CMAB) problem with fairness and privacy guarantees in a federated environment. We consider merit-based exposure as the desired fair outcome, which provides exposure to each action in proportion to the reward associated. We model the algorithm's effectiveness using fairness regret, which captures the difference between fair optimal policy and the policy output by the algorithm. Applying fair CMAB algorithm to each agent individually leads to fairness regret linear in the number of agents. We propose that collaborative -- federated learning can be more effective and provide the algorithm Fed-FairX-LinUCB that also ensures differential privacy. The primary challenge in extending the existing privacy framework is designing the communication protocol for communicating required information across agents. A naive protocol can either lead to weaker privacy guarantees or higher regret. We design a novel communication protocol that allows for (i) Sub-linear theoretical bounds on fairness regret for Fed-FairX-LinUCB and comparable bounds for the private counterpart, Priv-FairX-LinUCB (relative to single-agent learning), (ii) Effective use of privacy budget in Priv-FairX-LinUCB. We demonstrate the efficacy of our proposed algorithm with extensive simulations-based experiments. We show that both Fed-FairX-LinUCB and Priv-FairX-LinUCB achieve near-optimal fairness regret.

==> Plots/Agents.tex <==
% [3188.520293901566, 2341.131869558899, 2182.9453906995764, 1426.6962503216969, 1410.2518116239437, 1296.2869663935865]

% [3170.532045918757, 2684.13207162077, 1993.9996755662771, 1938.5856871359636, 1404.3444490200932, 1410.706385639031]

\begin{figure}[h!]
    \centering
    \begin{tikzpicture}[trim axis left, trim axis right]
        \begin{axis}[
            % width=\linewidth,
            height = 6cm,
    %             tick scale binop=\times,
    %             title={\ouralgo: FR vs. $\epsilon$},
    %             % ytick={0,0.5,1,1.5},
            xtick={2,4,6,8,10},
            xlabel={Agents ($m$)},
            xlabel near ticks,
            ylabel={Fairness Regret},
            ylabel near ticks,
            ymajorgrids=true,
            xmajorgrids=true,
            grid style=dashed,
            legend style={at={(1,1)},{column sep=0.01cm}},  
            legend entries={\small \ourprivalgo,\small \algoname},
    %             % every axis plot/.append style={thick}
        ]
                \addplot[color=myred,loosely dashed, every mark/.append style={solid, fill=gray},mark=square*]
                coordinates {
                (2, 2684.13207162077)
                (4, 1993.9996755662771)
                (6, 1938.5856871359636)
                (8, 1404.3444490200932)
                (10, 1410.706385639031)};
                
                \addplot[color=mytealdos,loosely dashed, every mark/.append style={solid, fill=gray},mark=star]    
                coordinates {
                (2, 2341.131869558899)
                (4, 2182.9453906995764)
                (6, 1426.6962503216969)
                (8, 1410.2518116239437)
                (10, 1296.2869663935865)};
            \end{axis}
        \end{tikzpicture}
\label{fig:agents}
% % \caption{$c{_{ij}},q_{i} \sim \mathcal{N}(\alpha=0.4,0.2)$ }
\caption{Fairness regret for \algoname\ and \ourprivalgo\ with respect to the number of agents $m$, observed at $T=100,000$ with $(\epsilon = 2, \delta = 0.1)$.}
\end{figure}

==> Plots/Epsilon.tex <==
% [3009.537541158756, 2022.1482217010616, 2161.8114335952987, 1383.9164497285542, 1632.1401226366554, 1224.2291907517565]

% [3027.814251030743, 3053.0032979190432, 2968.8011925361707, 2288.8568274001022, 2260.2942188295847, 1750.26074339728]

% [3145.1049759108437, 17766.264776730597, 17202.652187556832, 18474.28990623409, 16608.48790766844, 16698.873811438138]
\begin{figure}
    \centering
    \captionsetup[subfigure]{justification=centering}
    % Regret vs Rounds - Single vs Fed vs Pric
    
    \begin{subfigure}{0.5 \textwidth}
        \centering
        \begin{tikzpicture}[trim axis left, trim axis right]
            \centering
            \begin{axis}[
                % width=0.35 \textwidth,
                height = 5.5cm,
                % tick scale binop=\times,
        %             title={\ouralgo: FR vs. $\epsilon$},
        %             % ytick={0,0.5,1,1.5},
                xtick={0,25000,50000,75000,100000},
                xticklabel style = {font=\small,yshift=0.5ex},
                xlabel={Round ($t$)},
                scaled x ticks=false,
                xlabel near ticks,
                ytick={0,1000,2000,3000,4000,5000},
                ylabel={Fairness Regret},
                ylabel near ticks,
                xlabel style={font=\small},
                ylabel style={font=\small},
                ymax=5000,
                ymajorgrids=true,
                xmajorgrids=true,
                grid style=dashed,
                legend style={at={(0,1)},anchor=north west,{column sep=0.05cm},nodes={scale=0.75, transform shape}},  
                legend entries={B0,\ourprivalgo,\algoname},
                ticklabel style={font=\small},
        %             % every axis plot/.append style={thick}
            ]
                    \addplot[color=mygreen,dashdotted,line width=0.75pt]
                    coordinates {(0, 0.18) (1000, 161.92) (2000, 287.2) (3000, 394.42) (4000, 491.36) (5000, 580.5) (6000, 660.96) (7000, 737.12) (8000, 812.65) (9000, 883.57) (10000, 951.72) (11000, 1016.9) (12000, 1079.92) (13000, 1140.13) (14000, 1199.22) (15000, 1255.4) (16000, 1308.86) (17000, 1362.7) (18000, 1414.52) (19000, 1465.87) (20000, 1516.07) (21000, 1564.61) (22000, 1613.12) (23000, 1660.64) (24000, 1706.62) (25000, 1752.63) (26000, 1797.61) (27000, 1841.73) (28000, 1884.7) (29000, 1926.11) (30000, 1966.93) (31000, 2007.33) (32000, 2047.71) (33000, 2088.16) (34000, 2128.41) (35000, 2167.74) (36000, 2206.17) (37000, 2244.04) (38000, 2281.72) (39000, 2319.6) (40000, 2356.52) (41000, 2393.18) (42000, 2429.21) (43000, 2465.67) (44000, 2501.41) (45000, 2536.29) (46000, 2570.86) (47000, 2604.63) (48000, 2637.75) (49000, 2670.07) (50000, 2701.97) (51000, 2733.48) (52000, 2765.45) (53000, 2797.36) (54000, 2828.54) (55000, 2859.64) (56000, 2889.53) (57000, 2919.57) (58000, 2948.84) (59000, 2977.98) (60000, 3006.47) (61000, 3034.28) (62000, 3061.83) (63000, 3089.75) (64000, 3117.21) (65000, 3144.55) (66000, 3171.16) (67000, 3197.81) (68000, 3224.76) (69000, 3251.53) (70000, 3277.92) (71000, 3304.03) (72000, 3330.33) (73000, 3356.38) (74000, 3382.2) (75000, 3407.64) (76000, 3432.79) (77000, 3457.82) (78000, 3482.94) (79000, 3507.86) (80000, 3532.68) (81000, 3557.34) (82000, 3581.66) (83000, 3605.59) (84000, 3629.98) (85000, 3654.56) (86000, 3679.36) (87000, 3704.15) (88000, 3728.29) (89000, 3752.44) (90000, 3776.84) (91000, 3801.22) (92000, 3825.48) (93000, 3849.51) (94000, 3873.34) (95000, 3896.78) (96000, 3919.81) (97000, 3942.65) (98000, 3965.88) (99000, 3988.82)};
                    
                    \addplot[color=mytealtres,solid,line width=0.5pt]
                    coordinates {(0, 0.14) (1000, 165.52) (2000, 239.66) (3000, 298.15) (4000, 354.05) (5000, 409.18) (6000, 463.17) (7000, 501.16) (8000, 529.6) (9000, 558.35) (10000, 586.95) (11000, 613.82) (12000, 638.13) (13000, 662.16) (14000, 686.81) (15000, 711.79) (16000, 738.44) (17000, 765.28) (18000, 791.62) (19000, 818.41) (20000, 842.2) (21000, 864.52) (22000, 886.59) (23000, 908.71) (24000, 931.19) (25000, 953.38) (26000, 975.55) (27000, 997.68) (28000, 1019.89) (29000, 1038.22) (30000, 1056.81) (31000, 1075.21) (32000, 1093.5) (33000, 1111.42) (34000, 1129.07) (35000, 1146.63) (36000, 1163.94) (37000, 1182.07) (38000, 1201.55) (39000, 1221.09) (40000, 1240.66) (41000, 1260.47) (42000, 1282.29) (43000, 1304.26) (44000, 1325.98) (45000, 1347.56) (46000, 1367.01) (47000, 1385.8) (48000, 1404.51) (49000, 1423.01) (50000, 1441.33) (51000, 1458.82) (52000, 1476.22) (53000, 1493.45) (54000, 1510.69) (55000, 1527.62) (56000, 1544.53) (57000, 1561.51) (58000, 1578.09) (59000, 1594.47) (60000, 1610.88) (61000, 1626.75) (62000, 1642.76) (63000, 1658.15) (64000, 1672.57) (65000, 1686.99) (66000, 1701.48) (67000, 1715.93) (68000, 1730.73) (69000, 1745.67) (70000, 1760.13) (71000, 1774.72) (72000, 1788.96) (73000, 1803.11) (74000, 1817.1) (75000, 1830.83) (76000, 1844.02) (77000, 1856.1) (78000, 1868.16) (79000, 1880.23) (80000, 1892.42) (81000, 1903.85) (82000, 1915.13) (83000, 1926.65) (84000, 1938.15) (85000, 1950.26) (86000, 1962.43) (87000, 1974.63) (88000, 1986.66) (89000, 1998.9) (90000, 2011.4) (91000, 2023.95) (92000, 2036.47) (93000, 2049.07) (94000, 2062.5) (95000, 2076.18) (96000, 2089.73) (97000, 2103.03) (98000, 2116.19) (99000, 2129.16)};
                    \addplot[color=myred,dashed,line width=0.75pt]
                    coordinates {(0, 0.21) (1000, 97.09) (2000, 143.06) (3000, 186.2) (4000, 213.36) (5000, 238.76) (6000, 263.13) (7000, 297.42) (8000, 336.54) (9000, 375.9) (10000, 414.97) (11000, 450.43) (12000, 477.45) (13000, 503.58) (14000, 528.96) (15000, 555.36) (16000, 569.82) (17000, 583.64) (18000, 597.23) (19000, 611.12) (20000, 622.15) (21000, 631.45) (22000, 640.85) (23000, 650.12) (24000, 658.35) (25000, 664.54) (26000, 670.84) (27000, 677.15) (28000, 683.62) (29000, 690.81) (30000, 697.84) (31000, 704.94) (32000, 712.19) (33000, 719.71) (34000, 727.29) (35000, 734.98) (36000, 742.73) (37000, 750.97) (38000, 760.26) (39000, 769.46) (40000, 778.42) (41000, 787.58) (42000, 795.78) (43000, 803.94) (44000, 812.05) (45000, 820.12) (46000, 828.01) (47000, 835.66) (48000, 843.18) (49000, 850.75) (50000, 857.69) (51000, 863.75) (52000, 869.66) (53000, 875.56) (54000, 881.38) (55000, 885.91) (56000, 890.36) (57000, 894.87) (58000, 899.34) (59000, 904.14) (60000, 909.03) (61000, 913.84) (62000, 918.64) (63000, 924.01) (64000, 930.03) (65000, 936.19) (66000, 942.25) (67000, 948.29) (68000, 953.58) (69000, 958.88) (70000, 964.12) (71000, 969.49) (72000, 975.06) (73000, 980.57) (74000, 985.97) (75000, 991.26) (76000, 996.2) (77000, 1000.47) (78000, 1004.95) (79000, 1009.37) (80000, 1014.12) (81000, 1020.49) (82000, 1026.72) (83000, 1033.05) (84000, 1039.3) (85000, 1044.75) (86000, 1050.02) (87000, 1055.27) (88000, 1060.49) (89000, 1066.26) (90000, 1072.69) (91000, 1079.07) (92000, 1085.61) (93000, 1092.15) (94000, 1098.97) (95000, 1105.93) (96000, 1112.7) (97000, 1119.62) (98000, 1127.28) (99000, 1135.03)};
            \end{axis}
        \end{tikzpicture}
        \label{fig:rounds}
        \caption{ Exp 1 }
    \end{subfigure}

    % Regret vs Rounds - Communication Protocols
    
    \begin{subfigure}{0.5 \textwidth}
        \centering
        \begin{tikzpicture}[trim axis left, trim axis right]
            \begin{axis}[
                % width=\linewidth,
                height = 5.5cm,
                % tick scale binop=\times,
        %             title={\ouralgo: FR vs. $\epsilon$},
        %             % ytick={0,0.5,1,1.5},
                xtick={0,25000,50000,75000,100000},
                xticklabel style = {font=\small,yshift=0.5ex},
                xlabel={Round ($t$)},
                scaled x ticks=false,
                xlabel near ticks,
                ytick={0,1000,2000,3000,4000,5000},
                ylabel={Fairness Regret},
                ylabel near ticks,
                xlabel style={font=\small},
                ylabel style={font=\small},
                ymax=5000,
                ymajorgrids=true,
                xmajorgrids=true,
                grid style=dashed,
                legend style={at={(0,1)},anchor=north west,{column sep=0.05cm},nodes={scale=0.75, transform shape}},  
                legend entries={\ourprivalgo, B1, B2},
                ticklabel style={font=\small},
        %             % every axis plot/.append style={thick}
            ]
                    \addplot[color=mytealtres,solid,line width=0.5pt]
                    coordinates {(0, 0.14) (1000, 165.52) (2000, 239.66) (3000, 298.15) (4000, 354.05) (5000, 409.18) (6000, 463.17) (7000, 501.16) (8000, 529.6) (9000, 558.35) (10000, 586.95) (11000, 613.82) (12000, 638.13) (13000, 662.16) (14000, 686.81) (15000, 711.79) (16000, 738.44) (17000, 765.28) (18000, 791.62) (19000, 818.41) (20000, 842.2) (21000, 864.52) (22000, 886.59) (23000, 908.71) (24000, 931.19) (25000, 953.38) (26000, 975.55) (27000, 997.68) (28000, 1019.89) (29000, 1038.22) (30000, 1056.81) (31000, 1075.21) (32000, 1093.5) (33000, 1111.42) (34000, 1129.07) (35000, 1146.63) (36000, 1163.94) (37000, 1182.07) (38000, 1201.55) (39000, 1221.09) (40000, 1240.66) (41000, 1260.47) (42000, 1282.29) (43000, 1304.26) (44000, 1325.98) (45000, 1347.56) (46000, 1367.01) (47000, 1385.8) (48000, 1404.51) (49000, 1423.01) (50000, 1441.33) (51000, 1458.82) (52000, 1476.22) (53000, 1493.45) (54000, 1510.69) (55000, 1527.62) (56000, 1544.53) (57000, 1561.51) (58000, 1578.09) (59000, 1594.47) (60000, 1610.88) (61000, 1626.75) (62000, 1642.76) (63000, 1658.15) (64000, 1672.57) (65000, 1686.99) (66000, 1701.48) (67000, 1715.93) (68000, 1730.73) (69000, 1745.67) (70000, 1760.13) (71000, 1774.72) (72000, 1788.96) (73000, 1803.11) (74000, 1817.1) (75000, 1830.83) (76000, 1844.02) (77000, 1856.1) (78000, 1868.16) (79000, 1880.23) (80000, 1892.42) (81000, 1903.85) (82000, 1915.13) (83000, 1926.65) (84000, 1938.15) (85000, 1950.26) (86000, 1962.43) (87000, 1974.63) (88000, 1986.66) (89000, 1998.9) (90000, 2011.4) (91000, 2023.95) (92000, 2036.47) (93000, 2049.07) (94000, 2062.5) (95000, 2076.18) (96000, 2089.73) (97000, 2103.03) (98000, 2116.19) (99000, 2129.16)};
                    \addplot[color=teal,dashdotted,line width=0.75pt]
                    coordinates {(0, 0.12) (1000, 175.92) (2000, 305.93) (3000, 434.43) (4000, 560.78) (5000, 668.58) (6000, 747.35) (7000, 793.72) (8000, 841.06) (9000, 888.09) (10000, 933.67) (11000, 977.13) (12000, 1019.41) (13000, 1060.8) (14000, 1101.6) (15000, 1141.97) (16000, 1181.67) (17000, 1221.17) (18000, 1259.49) (19000, 1296.86) (20000, 1333.48) (21000, 1369.27) (22000, 1406.29) (23000, 1442.27) (24000, 1478.35) (25000, 1514.06) (26000, 1550.0) (27000, 1586.19) (28000, 1621.93) (29000, 1657.82) (30000, 1693.15) (31000, 1726.54) (32000, 1760.68) (33000, 1794.42) (34000, 1827.82) (35000, 1860.28) (36000, 1893.32) (37000, 1925.74) (38000, 1958.47) (39000, 1990.85) (40000, 2023.0) (41000, 2054.65) (42000, 2086.31) (43000, 2117.41) (44000, 2148.68) (45000, 2179.24) (46000, 2209.83) (47000, 2239.89) (48000, 2269.64) (49000, 2299.43) (50000, 2328.82) (51000, 2358.27) (52000, 2387.84) (53000, 2417.68) (54000, 2446.68) (55000, 2475.92) (56000, 2505.08) (57000, 2533.42) (58000, 2562.07) (59000, 2590.61) (60000, 2619.72) (61000, 2647.66) (62000, 2675.25) (63000, 2697.91) (64000, 2707.03) (65000, 2716.08) (66000, 2725.17) (67000, 2734.24) (68000, 2743.41) (69000, 2752.49) (70000, 2761.42) (71000, 2770.21) (72000, 2779.19) (73000, 2788.21) (74000, 2797.17) (75000, 2806.05) (76000, 2814.84) (77000, 2823.66) (78000, 2832.43) (79000, 2841.27) (80000, 2850.02) (81000, 2858.75) (82000, 2867.55) (83000, 2876.39) (84000, 2885.17) (85000, 2893.79) (86000, 2902.31) (87000, 2911.02) (88000, 2919.61) (89000, 2928.24) (90000, 2936.85) (91000, 2945.47) (92000, 2954.22) (93000, 2962.95) (94000, 2971.51) (95000, 2980.03) (96000, 2988.69) (97000, 2997.11) (98000, 3005.57) (99000, 3014.11)};
                    \addplot[color=orange,dashed,line width=0.75pt]
                    coordinates {(0, 0.15) (1000, 149.7) (2000, 197.03) (3000, 239.52) (4000, 292.27) (5000, 346.18) (6000, 398.76) (7000, 448.92) (8000, 496.73) (9000, 543.58) (10000, 590.41) (11000, 636.87) (12000, 682.76) (13000, 722.25) (14000, 741.64) (15000, 761.12) (16000, 780.5) (17000, 800.46) (18000, 820.57) (19000, 840.26) (20000, 859.98) (21000, 879.85) (22000, 900.22) (23000, 920.4) (24000, 940.03) (25000, 959.89) (26000, 977.25) (27000, 992.42) (28000, 1007.59) (29000, 1022.61) (30000, 1037.92) (31000, 1052.96) (32000, 1067.9) (33000, 1082.89) (34000, 1097.81) (35000, 1113.0) (36000, 1128.17) (37000, 1143.13) (38000, 1158.61) (39000, 1173.74) (40000, 1188.83) (41000, 1204.13) (42000, 1219.27) (43000, 1234.56) (44000, 1250.06) (45000, 1265.02) (46000, 1280.08) (47000, 1294.93) (48000, 1309.58) (49000, 1324.11) (50000, 1338.63) (51000, 1353.04) (52000, 1365.15) (53000, 1376.66) (54000, 1388.45) (55000, 1400.34) (56000, 1411.98) (57000, 1423.81) (58000, 1435.53) (59000, 1447.43) (60000, 1459.14) (61000, 1470.79) (62000, 1482.26) (63000, 1493.81) (64000, 1505.33) (65000, 1517.11) (66000, 1528.66) (67000, 1540.09) (68000, 1551.75) (69000, 1563.1) (70000, 1574.44) (71000, 1586.04) (72000, 1597.57) (73000, 1608.94) (74000, 1620.18) (75000, 1631.41) (76000, 1642.74) (77000, 1654.0) (78000, 1665.37) (79000, 1676.61) (80000, 1688.19) (81000, 1699.5) (82000, 1710.9) (83000, 1722.37) (84000, 1733.79) (85000, 1745.02) (86000, 1756.24) (87000, 1767.57) (88000, 1778.69) (89000, 1790.03) (90000, 1801.19) (91000, 1812.45) (92000, 1823.75) (93000, 1834.88) (94000, 1846.12) (95000, 1857.7) (96000, 1868.9) (97000, 1880.35) (98000, 1891.74) (99000, 1903.45)};
            \end{axis}
        \end{tikzpicture}
        \caption{ Exp 2 }
        \label{fig:comm}
    \end{subfigure}

    
    \caption{Round-wise per agent regret trend comparison between (a) Different algorithms; (b) \ourprivalgo\ with various communication protocols}
    \label{fig:epsilon}
\end{figure}

==> Subparts/lemma_proof.tex <==
With the help of the above lemmas, we can easily prove the instantaneous regret \(FR_t^i\). 
\begin{lemma} \label{lemma:Instanteous Regret}
    For the \algoname \  algorithm, the instantaneous regret for any agent \(i\) is given by,
    \begin{align*}
        {FR}_{t}^{i} = \sum_{a \in \altmathcal{D}} \left| \pi_{t}^{i} - \pi_{*}^{i} \right| \leq \frac{4L\sqrt{\beta_{t}}}{\gamma}\mathbb{E}_{a \sim \pi_{t}^{i} } \left\|x_{t}^i (a) \right\|_{(V_t^{i})^{-1}}
    \end{align*}
\end{lemma}
\begin{proof}
\allowdisplaybreaks
\begin{align*}
    {FR}_{t}^{i} &= \sum_{a\in \altmathcal{D}} \left| \frac{f^i(\theta^{*}x_{t}^i (a))}{\sum_{a^{'} \in \altmathcal{D}} f^i(\theta^{*}x_{t}^i (a^{\prime}))} - \frac{f^i(\theta^{i}_{t}x_{t}^i (a))}{\sum_{a^{'} \in \altmathcal{D}} f^i(\theta^{i}_{t}x_{t}^i (a^{\prime}))} \right| \\
    &= \sum_{a} \left| \frac{f^i(\theta^{*}x_{t}^i (a)) \sum_{a^{'}} f^i(\theta^{i}_{t}x_{t}^i (a^{\prime})) - f^i(\theta^{i}_{t}x_{t}^i (a)) \sum_{a^{'}} f^i(\theta^{*}x_{t}^i (a^{\prime}))}{\sum_{a^{'}} f^i(\theta^{i}_{t}x_{t}^i (a^{\prime})) \sum_{a^{'}} f^i(\theta^{*}x_{t}^i (a^{\prime}))} \right| \\
    & \\
    &= \sum_{a}  \frac{ \left| \splitfrac{f^i(\theta^{*}x_{t}^{i} (a)) \sum_{a^{'}} \left( f^i(\theta^{i}_{t}x_{t}^i (a^{\prime})) -  f^i(\theta^{*}x_{t}^i (a^{\prime})) \right)}{+\left( f^i(\theta^{*}x_{t}^{i} (a)) - f^i(\theta^{i}_{t}x_{t}^{i} (a)) \right) \sum_{a^{'}} f^i(\theta^{*}x_{t}^i (a^{\prime}))} \right|}{\sum_{a^{'}} f^i(\theta^{i}_{t}x_{t}^i (a^{\prime})) \sum_{a^{'}} f^i(\theta^{*}x_{t}^i (a^{\prime}))}  \\
    & \\
    &\leq \sum_{a}  \frac{  \splitfrac{ \left|f^i(\theta^{*}x_{t}^{i} (a)) \sum_{a^{'}} \left( f^i(\theta^{i}_{t}x_{t}^i (a^{\prime})) -  f^i(\theta^{*}x_{t}^i (a^{\prime})) \right) \right|}{+\left|\left( f^i(\theta^{*}x_{t}^{i} (a)) - f^i(\theta^{i}_{t}x_{t}^{i} (a)) \right) \sum_{a^{'}} f^i(\theta^{*}x_{t}^i (a^{\prime})) \right|} }{\sum_{a^{'}} f^i(\theta^{i}_{t}x_{t}^i (a^{\prime})) \sum_{a^{'}} f^i(\theta^{*}x_{t}^i (a^{\prime}))} \\
    &\leq  \frac{ 2\sum_{a} \left|  f^i(\theta^{*}x_{t}^{i} (a)) - f^i(\theta^{i}_{t}x_{t}^{i} (a))  \right|}{\sum_{a^{'}} f^i(\theta^{i}_{t}x_{t}^i (a^{\prime}))} \\
    &= 2\sum_{a} \frac{\pi_{t}^{i}}{f^i(\theta^{i}_{t}x_{t}^{i} (a))} \left|  \begin{aligned}
        &f^i(\theta^{*}x_{t}^{i} (a)) - f^i(\hat{\theta^{i}_{t}}x_{t}^{i} (a)) \\
        &+ f^i(\hat{\theta^{i}_{t}}x_{t}^{i} (a)) - f^i(\theta^{i}_{t}x_{t}^{i} (a)) 
    \end{aligned} \right| \\
    &\leq \frac{2L}{\gamma} \mathbb{E}_{a  \sim \pi_{t}^{i} } \left[ 
    \begin{aligned}
        &\left\| \theta^{*} - \hat{\theta^{i}_{t}} \right\|_{V_t^{i}} \left\| x_{t}^{i} (a) \right\|_{(V_t^{i})^{-1}} \\
        &+ \left\| \hat{\theta^{i}_{t}} - \theta^{i}_{t} \right\|_{V_t^{i}} \left\| x_{t}^{i} (a) \right\|_{(V_t^{i})^{-1}}
    \end{aligned} \right] \\
    &\leq \frac{4L\sqrt{\beta_{t}}}{\gamma}\mathbb{E}_{a \sim \pi_{t}^{i} } \left\|x_{t}^i (a)\right\|_{(V_t^{i})^{-1}}
\end{align*}
\end{proof}

==> Subparts/related_works.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Related Works}\label{sec:rel_work}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% MABs
\textbf{MAB and Contextual Bandits.} The field of multi-armed bandits (MABs) has been extensively studied in the literature (\cite{bams/1183517370}, \cite{LAI19854}, \cite{auer}). Our work considers the contextual bandit, which is a more general bandit framework. Our work builds on the LinUCB algorithm which was introduced in \cite{li2010contextual} and later improved by \cite{NIPS2011_e1d5be1c}.

\textbf{Differential Privacy.} Our work leverages differential privacy, first introduced by \cite{dwork2006calibrating}, a rigorous mathematical notion for privacy that encapsulates the requirement that the probability of output should have minimal changes for neighboring input datasets. \cite{privatecontinual} and \cite{dwork2010differential} introduced the notion of differential privacy under continual observation using a \textbf{tree-based algorithm}. The algorithm leverages the tree structure to privatize partial sums of \(n\) observations using a maximum of \(\log(n)\) noise term additions. This method has seen utilization across several online learning problems (\cite{tossou2016algorithms}, \cite{NIPS2013_c850371f}, \cite{kairouz2021advances}, \cite{jain2012differentially}). 

More recently, a lot of work has been done in differentially private MAB settings. \cite{mishra2015nearly}, \cite{hu2022near}, \cite{azize2022when} provide differential privacy guarantees for the single-player stochastic bandit setting. \cite{shariff2018differentially} studies differential privacy in a contextual bandit setting and is more closely related to our setting, but is limited to a single learning agent. \cite{he2022a} and \cite{da2022nearoptimal} conversely studies the contextual bandit problem for federated learning agents but in a non-private setting. The notion of differential private federated bandits has been studied in \cite{liu2022federated} and \cite{ECML}, but our work is most closely related to the important work of \cite{shariff2018differentially} and \cite{dubey2020differentially}, extending it for non-traditional bandit optimization objectives.

\textbf{Fairness in Bandits.} Algorithmic fairness has been extensively studied for machine learning algorithms, including online learning (\cite{hardt2016equality}, \cite{jang2022group}). The purpose is to evaluate the efficacy of algorithms in terms of fairness from philosophical and societal standpoints by developing quantifiable definitions of fairness. There have been advancements in fair bandit algorithms in recent years. 

\cite{NIPS2016_eb163727} provides bandit fairness by ensuring that a better arm is always chosen with at least the same likelihood as a worse arm. \cite{chen2020fair}, \cite{li2022efficient} and \cite{patil2020achieving} ensures minimum exposure for arms. Meanwhile, \cite{grazzi2022group} provides group fairness in the contextual bandit paradigm. Our definition of fairness focuses on the proportionality of exposure and merit (\cite{NEURIPS2019_9e82757e}) for the arms in the bandit problem. \cite{wang2021fairness} works with the same notion of fairness as our work and provides algorithmic solutions but is limited to the single-player setting.

To the best of our knowledge, our work is the premiere work to generalize fair bandits into a federated setting in addition to being the first work to incorporate the notion of both fairness and privacy simultaneously for the bandit problem. 



% Recent Work - 
% \begin{itemize}
%     % \item \cite{hu2022near} - DP in Thompson sampling for stochastic bandits, single-player setting (reward observations are private values). (UAI 2022) - done
%     % \item \cite{li2022efficient} - Fairness constraints (minimum share) in restless bandits. (UAI 2022)
%     % \item \cite{liu2022federated} - Differential privacy in contextual federated setting for clusters. (UAI 2022) - done
%     % \item \cite{he2022a} - Federated Contextual Bandits with asynchronous communication. (NO DP or fairness) (NIPS 2022)
%     % \item \cite{azize2022when} - DP in stochastic bandit setting (no federated, no fairness). (NIPS 2022) - done
%     \item \cite{grazzi2022group} - Group Fairness in Linear Contextual Bandits. Picking the 
%  best arm based on relative ranking within sensitive groupings. (NIPS 2022)
%     % \item \cite{da2022nearoptimal} - Federated contextual bandits. (NIPS 2022)
%     % \item \cite{pmlr-v162-chowdhury22a} - DP in contextual bandits. (ICML 2022)
%     \item \cite{patil2020achieving} Fairness of minimum exposure in bandits. (AAAI 2020)
% \end{itemize}

% Important Related work - 

% \begin{itemize}
%     \item \textbf{DP}
%     \item \cite{mishra2015nearly} - Differentially private algorithms for stochastic MABs. (UAI 2015)
%     \item \cite{shariff2018differentially} - Differentially Private LinUCB based algorithm, for single player contextual bandit setting. (NIPS 2018)
%     \item \textbf{DP + Federated}
%     \item \cite{dubey2020differentially} Federated DP contextual Bandits.
%     \item \cite{} ECML paper
%     \item \textbf{Fairness}
%     \item \cite{wang2021fairness} FairX bandit algorithm. (ICML 2021)
%     \item \cite{NEURIPS2019_9e82757e} Merit-based fairness  of exposure constraints introduced. (NIPS 2019)
%     \item \cite{NIPS2016_eb163727} Introduced the study of fairness in multi-armed bandit problems, a worse arm should not be more likely to be picked than a better arm. (NIPS 2016)
% \end{itemize}

